An abstract approximation tool for mixed-dimensional and equidimensional modeling

Many coupled problems in engineering and science can be described by elliptic partial differential equations on adjacent domains, where the coupling can be considered either as a thin equidimensional overlap between the model domains, or as a lower-dimensional interface. Thereby we distinguish equidimensional and mixed-dimensional models of the same system, and the relationship between these modeling approaches is of natural interest. In this paper, we construct an overlapping open cover for a class of simplicial geometries and construct a bounded cochain map from the simplicial de Rham complex to the \v{C}ech-de Rham complex associated with the overlapping cover. Thus, we establish an isomorphism between simplicial de Rham complexes (i.e. functions and forms on mixed-dimensional partitions and their differentials) and subcomplexes of \v{C}ech-de Rham complexes (i.e. functions and forms on equidimensional partitions and their differentials), which serves as an abstract approximation tool for comparing mixed-dimensional problems to the equidimensional version of the same problem.

==> extra.tex <==
%The trace operator plays an important role in the construction of the cochain maps. The trace operator decreases the regularity, i.e. the range of the trace operator $\tr(H^1(\Omega)) = H^{1/2}(\partial \Omega)$ is not in $H^1(\partial \Omega)$. We are interested in subcomplexes of the Sobolev-de Rham complex where the trace is also in $H\Lambda^k$ on its boundary:
%\begin{equation}
%H\Lambda^k(\Omega, \tr_{\partial}) = \{\alpha \in H\Lambda^k(\Omega) : \tr \; \alpha \in H\Lambda^k(\partial \Omega) \} \label{eq: enhanced regularity sdr}
%\end{equation}

%both with coefficients in the Sobolev-de Rham complex $H\Lambda^\bullet$.

%Rewrite to account for cutting section 3
%We restrict the exposition to geometries where the number of manifolds $\Omega_i$ in each codimension $p$ corresponds one-to-one with the number of non-empty intersections $U_i$ of degree $p$. Because of this correspondence, we can by assumption index the $n$-simplices $\{\Omega_i\}_{i \in \Ic}$ and the open cover $\Uc = \{U_i\}_{i \in \Ic}$ by the same index set $\Ic$.
%Let $\alpha \in \Sc^{p,q}$ with components $\alpha_i$ for each $i \in \Ic^p$. We write $(i,j) \in \Ic_i^{p+s}$, where $i$ and $j$ are disjoint multi-indices with $j \in \Ic^{s-1}$, and $(i,m) \in \Ic^n$.
%\textcolor{blue}{
%\begin{align*}
%U_i = \cup_j \tilde{U}_i^j\\
%\tilde{U}_i^{\varnothing}=\tilde{U}_i
%\end{align*}
%}

%\begin{figure}[htb]
%    \centering 
%   \includegraphics[scale=0.75]{figure2.jpg}
%    \caption{On the left, we have a one-dimensional manifold $\Omega_i$ with codimension one. On the right, we have the corresponding $\Tilde{U}_i$. $\Omega_i$ is a submanifold of $\Tilde{U}_i$, and $\phi$ is the restriction onto $\Omega_i$. The induced pullback is then a mapping of differential forms from $\Omega_i$ onto $\Tilde{U}_i$, where the differential forms are constant along the lines normal to $\Omega_i$.
%    }
%    \label{fig: pullback}
%\end{figure}


%In addition, there are surjective maps $\phi_{ij}: \Tilde U_{ij} \to \Omega_{ij}$, which induces pullbacks $\phi_{ij}^*: \Lambda^\bullet(\Omega_{ij}) \to \Lambda^\bullet(\Tilde{U}_{ij})$. These pullbacks maps a differential form on the interface $\Omega_{ij}$ to a differential form on the intersection $U_{ij}$, which is constant in the direction normal to the interface. We also have a constant map $\phi_{123}^*: \Lambda^0(\Omega_{123}) \to \Lambda^{0}(\Tilde U_{123})$, where a constant value $c \in \Omega_{123}$ is mapped to a constant function $c|_{U_{123}}$.

Old abstract:
\begin{abstract}
For a class of simplicial geometries, we construct an open cover where each lower-dimensional simplex of codimension $p$ is covered by an intersection of $p+1$ open sets in the open cover. We construct an injective cochain map from the simplicial de Rham complex to the \v{C}ech-de Rham complex of the open cover. Both the double complexes have coefficients in $L^2$, and the cochain map we construct is between the respective domain complexes.

The image of the cochain map will be an embedding of the simplicial de Rham complex, realizing it as a subcomplex of the \v{C}ech-de Rham complex. The simplicial de Rham complex and the \v{C}ech-de Rham complex represent mixed-dimensional and equidimensional coupled problems, respectively. Thus, we establish a structure-preserving relationship between certain mixed-dimensional problems and their equidimensional counterparts.
\end{abstract}

%\subsection{Bounded cochain projections}
%The cochain map $\Xi$ defines an embedding $\Xi^\bullet(\Sc) \subset \Ac^\bullet$. Thus, we can view the embedded simplicial de Rham complex as a subcomplex of the \v{C}ech-de Rham complex. If one construct bounded cochain projections from the \v{C}ech-de Rham complex to the subcomplex defined by $\Xi$, following the theory of FEEC on obtains an approximation theory for Hodge-Laplace problems on the two respective double complexes.
